One DSL to Rule Them All: IDE-Assisted Code Generation for Agile Data Analysis

Data analysis is at the core of scientific studies, a prominent task that researchers and practitioners typically undertake by programming their own set of automated scripts. While there is no shortage of tools and languages available for designing data analysis pipelines, users spend substantial effort in learning the specifics of such languages/tools and often design solutions too project specific to be reused in future studies. Furthermore, users need to put further effort into making their code scalable, as parallel implementations are typically more complex. We address these problems by proposing an advanced code recommendation tool which facilitates developing data science scripts. Users formulate their intentions in a human-readable Domain Specific Language (DSL) for dataframe manipulation and analysis. The DSL statements can be converted into executable Python code during editing. To avoid the need to learn the DSL and increase user-friendliness, our tool supports code completion in mainstream IDEs and editors. Moreover, DSL statements can generate executable code for different data analysis frameworks (currently we support Pandas and PySpark). Overall, our approach attempts to accelerate programming of common data analysis tasks and to facilitate the conversion of the implementations between frameworks. In a preliminary assessment based on a popular data processing tutorial, our tool was able to fully cover 9 out of 14 processing steps for Pandas and 10 out of 16 for PySpark, while partially covering 4 processing steps for each of the frameworks.

==> latex mirror/011-abstract.tex <==
Data analysis is at the core of scientific studies, a prominent task
that researchers and practitioners typically undertake by programming
their own set of automated scripts. While there is no shortage of
tools and languages available for designing data analysis pipelines,
users spend substantial effort in learning the specifics of such languages/tools
and often design solutions too project specific to be reused in future
studies. Furthermore, users need to put further effort into making
their code scalable, as parallel implementations are typically more
complex.

We address these problems by proposing an advanced code recommendation
tool which facilitates developing data science scripts. Users formulate
their intentions in a human-readable Domain Specific Language (DSL)
for dataframe manipulation and analysis. The DSL statements can be
converted into executable Python code during editing. To avoid the
need to learn the DSL and increase user-friendliness, our tool supports
code completion in mainstream IDEs and editors. Moreover, DSL statements
can generate executable code for different data analysis frameworks
(currently we support Pandas and PySpark). Overall, our approach attempts
to accelerate programming of common data analysis tasks and to facilitate
the conversion of the implementations between frameworks.

In a preliminary assessment based on a popular data processing tutorial,
our tool was able to fully cover 9 out of 14 processing steps for
Pandas and 10 out of 16 for PySpark, while partially covering 4 processing
steps for each of the frameworks.




==> latex mirror/040-evaluation.tex <==

\section{Preliminary Evaluation} \label{sec:Evaluation}

A proper evaluation of the usefulness of our approach would require
a well-designed user study with a sufficient number of participants.
Due to time constrains, we refrain from performing such analysis and
focus instead on assessing the coverage of our initial DSL implementation.
To that aim, in this preliminary evaluation we answer the following
question: Given a real-usage scenario, what fraction of the analysis
and data processing steps are covered by our current DSL design?

We first need to select a scenario that represents a typical data
analysis task. Due to the popularity and demand for data analysis
in current scientific landscape, tutorials are very common in the
web. For our evaluation, we select a popular DataCamp tutorial ``Apache
Spark Tutorial: ML with PySpark''\footnote{\href{https://www.datacamp.com/community/tutorials/apache-spark-tutorial-machine-learning}{https://www.datacamp.com/community/tutorials/apache-spark-tutorial-machine-learning}}
that provides a high-quality use-case for using PySpark dataframes
for data processing and data analysis. This tutorial has multiple
topics, ranging from Spark installation to the application of conventional
machine-learning methods for Big Data. For this initial assessment,
we focus only on the topics within the scope targeted by our DSL:
data exploration and data pre-processing. The two topics in this tutorial
contain a total of 16 \textit{processing steps}. We define a processing
step loosely as the smallest part of the code that can be executed
on its own (typically single-liners), or in a single block of code
in this tutorial.

To evaluate our DSL in context of Spark, we use unchanged source code
from the tutorial. For Pandas, we manually translate each processing
step into Pandas code, which yields only 14 processing steps, as some
steps (such as creating RDDs to populate dataframes) are specific
to PySpark. We do not use (another) tutorial directly for Pandas as
it was impossible to find a tutorial with similar purpose/scenario
as to the one for Spark. Moreover, many introductory tutorials for
Pandas explain functions related to selecting individual values (e.g.
\texttt{.loc} and \texttt{.iloc}), and functions related to the (row)
index data structure of Pandas. Such functions make Pandas code fundamentally
difficult to translate to other programming paradigms or frameworks
(e.g. SQL, Spark), and typically make the code non-scalable. In our
scenario, we assume that a developer considers the scenario of massive
data sets and will avoid such functions right from the onset. 

In our evaluation we attempt to express a basic processing step with
our DSL. For each such step, we estimate whether it can be expressed
in the DSL completely, whether DSL needs additional (Python) code,
whether we need to substantially change the generated code, or if
our DSL cannot express this step at all. We present in Table~\ref{tab:results_evaluation}
the aggregated results of this initial assessment. Overall, our DSL
fully covers 64.2\% of Pandas processing steps and 62.5\% of PySpark
processing steps in the tutorial. In 4 processing steps for Pandas
and PySpark, the translated code did not completely match the expected
goal and users would have to add Python code (either as new parameters
or function call) to fulfill their initial intention. We find no case
where the generated code needs to be rewritten but three processing
steps (one in Pandas and two in PySpark) could not be expresed or
translated by our DSL (see NS in Table \ref{tab:results_evaluation}). 

\begin{table}
\caption{\label{tab:results_evaluation}Results of our DSL coverage assessment
for Pandas and PySpark code translation. }

\begin{tabular}{lll}
\toprule 
Category & Pandas & PySpark\tabularnewline
\midrule 
Fully translated (FT) & 9/14 (64.2\%) & 10/16 (62.5\%)\tabularnewline
Code added (CA) & 4/14 (28.5\%) & 4/16 (25.0\%)\tabularnewline
Code modified (CM) & 0/14 (0.0\%) & 0/16 (0.0\%)\tabularnewline
DSL not suitable (NS) & 1/14 (7.1\%) & 2/16 (12.5\%)\tabularnewline
\bottomrule
\end{tabular}
\end{table}
In Table~\ref{tab:examples_translation}, we detail the processing
steps our DSL fail to cover in its completion (CA) or could not support
at all (NS). From the 11 partially failed steps, 6 were only covered
by a similarly equivalent function (L1). In this particular case,
our DSL generated the code to retrieve the top N rows in a dataframe
through the \texttt{head} function call, while in the tutorial the
\texttt{show} function is preferred. Both functions are similar in
practice, but \texttt{show} prints the top N rows in the standard
output, while \texttt{head} returns top N rows as a new dataframe.
In another case (L2), when sorting a dataframe, our DSL assumes the
sorting in the ascending order, hence omitting the optional parameter
for descending sorting (\texttt{ascending=False}). The L3 evidences
one limitation of our DSL, the lack of context awareness. In the current
implementation, the DSL does not index or complete code from functions
defined by the programmer and hence should not be used as a code recommender.
The last case (L4), is the support for lambda functions not yet implemented
in our tool. 

\begin{table*}
\caption{\label{tab:examples_translation}Examples of DSL limitation in fully
translating our studied tutorial into PySpark code. The ``Cat''
column references the categories of Table \ref{tab:examples_translation}.
The expected code written in \textbf{\textit{\textcolor{red}{red}}}
and bold is currently not supported by our DSL.}

\small

\begin{tabular}{lllllll}
\toprule 
ID & Cat. & Limitation & DSL code (\texttt{\#\#} is omitted) & Generated code & Expected generated code & \#\tabularnewline
\midrule 
L1 & CA & Target function not supported & on df: return top\_N 10 & df.head(10) & df.\textbf{\textit{\textcolor{red}{show}}}(10) & 6\tabularnewline
L2 & CA & Parameter not supported & on df : sort\_by col & df.sort('col') & df.sort('col', \textbf{\textit{\textcolor{red}{ascending=False}}}) & 2\tabularnewline
L3 & NS & Custom user-functions not supported & -- & -- & df = \textbf{\textit{\textcolor{red}{convertColumn}}}(df, columns,
FloatType()) & 2\tabularnewline
L4 & NS & Lambda functions not supported & -- & -- & df = rdd.\textbf{\textcolor{red}{\emph{apply}}}\textbf{\textcolor{red}{(}}\textbf{\textcolor{red}{\emph{lambda}}}\textbf{\textcolor{red}{{}
}}\textbf{\textcolor{red}{\emph{x}}}\textbf{\textcolor{red}{: }}\textbf{\textcolor{red}{\emph{x}}}\textbf{\textcolor{red}{{}
/ 10).}}\textbf{\textcolor{red}{\emph{toDF}}}\textbf{\textcolor{red}{()}} & 1\tabularnewline
\bottomrule
\end{tabular}
\end{table*}



==> latex mirror/050-related_work.tex <==

\section{Related Work} \label{sec:Related-Work}

Domains relevant to our work are \emph{low-code data analysis}, \emph{accelerated
scripting and coding}, and \emph{Domain Specific Languages}.

\emph{Low-code data analysis}. Multiple research fields tackle the
challenge of making the process of data analysis and transformation
more user-friendly and accelerating scripting and automation of processing.
The essential directions are: visual analytics \citep{macinnes2010visualclassification},
mixed-initiative systems \citep{horvitz1999principles}, \citep{makonin2016mixedinitiative},
facilitating user involvement in the data analysis or processing activities
\citep{doan2017humanintheloop}, \citep{rahman2018icarusminimizing},
learning data transformations by examples \citep{le2014flashextract},
\citep{smith2016mapreduce}, \citep{jin2017foofahtransforming}, \citep{raza2017automated},
and data wrangling in various flavors \citep{raman2001potters}, \citep{kandel2011wrangler},
\citep{stonebraker2013datacuration}, \citep{heer2015predictive},
\citep{rahman2018icarusminimizing}.

Data wrangling (or data munging) refers to the process of interactive
data transformations on structured or unstructured data. The most
mature tool in this domain is Wrangler \citep{kandel2011wrangler}
which was commercialized by Trifacta \citep{machlis2016datawrangling},
and recently offered by Google as the Google Cloud service \citep{gogle2017clouddataprep}.
Another popular tool is OpenRefine \citep{verborgh2013usingopenrefine}
(originally GoogleRefine) which allows batch processing of tabular
data by menu selection and a Domain Specific Language (DSL) named
GREL. Albeit similar to Wrangler, it has more restricted functionality
and offers no support for very large data sets.

The concept behind these tools is Predictive Interaction \citep{heer2015predictive}.
Its key elements are: (i) real-time preview of effects of code on
a processed data set, (ii) code recommendations based on the context
of user interactions and data, and (iii) a DSL to describe data transformations
in a way easily accessible to users. A disadvantage of the Wrangler
tool is the fact that it is a closed (and commercial) eco-system.
This creates a serious barrier for interoperability with mainstream
libraries or frameworks. Moreover, its DSL has a limited expressiveness
(focusing on data preparation only), and extending this DSL requires
developing User Defined Functions.

Learning data transformations by examples \citep{le2014flashextract},
\citep{smith2016mapreduce}, \citep{jin2017foofahtransforming}, \citep{raza2017automated}
is a special case of the program synthesis techniques. Such approaches
(while still immature) offer a promise to greatly facilitate complex
data analysis, especially for users with no or little programming
skills. The (quite sophisticated) methods here include constraint-based
program synthesis, program sketching \citep{solar-lezama2008program},
version space algebra \citep{le2014flashextract,gulwani2011automating},
or searching in a state space graph \citep{jin2017foofahtransforming}.
In context of data extraction, transformation, and analysis, several
interesting applications have been proposed \citep{gulwani2016programming},
including extracting relations from spreadsheets \citep{barowy2015flashrelate},
data transformations \citep{jin2017foofahtransforming}, or synthesizing
regular expressions. So far, only the FlashFill approach \citep{gulwani2015automating}
has been practically relevant and available to many users (as a component
of Excel 2013 and \emph{ConvertFrom-String} cmdlet in PowerShell).
We consider program synthesis as a possible extension of our work.

\emph{Accelerating scripting and coding} (and as a special case, end-user
development/end-user programming) comprises a multitude of approaches
from software engineering. The most visible progress in this category
stems from novel programming languages, introduction of software processes
such as Scrum, proliferation of software testing, and advances in
development tools (including Intelligent Development Environments,
or syntax/error checkers). Nevertheless, the impact of the individual
measures on programmers\textquoteright{} productivity is hard to measure.
Other noteworthy approaches include program synthesis (discussed above),
visual programming via dataflow languages \citep{johnston2004advances},
block programming languages \citep{bau2017learnable}, and Domain
Specific Languages (DSLs) \citep{fowler2010domainspecific,kosar2016domainspecific}
(discussed below), or more generally Language-Oriented Programming
\citep{felleisen2015theracket}.

In the context of data analysis, dataflow languages \citep{johnston2004advances,gotze2016rewriting}
have gained some popularity via tools such as \citep{2018top21} or
KNIME \citep{berthold2008knimethe}. Such approaches can greatly accelerate
creation of small data processing pipelines and have also proven suitable
for educational purposes. On the other hand, they tend to slow down
more experienced programmers (even smallest operation like \textquotedblleft +\textquotedblright{}
must be selected from menu/palette and connected to other blocks),
do not provide an intuitive support for controls structures, and lack
interoperability with other tools or libraries. For these reasons,
they are rarely used in larger projects.

\emph{Domain Specific Languages} (DSLs) \citep{fowler2010domainspecific},
\citep{kats2010thespoofax}, \citep{dejanovic2017textxa}, have proven
useful in a multitude of medium to large-scale projects by introducing
highly readable and concise code with support for higher-level operations.
While the underlying ``theory'' and scientific interest is still
modest \citep{kats2010thespoofax}, \citep{felleisen2015theracket},
\citep{gupta2015languagebased}, DSLs are becoming increasingly popular
in industry (for example, the industrial-grade database management
system SAP HANA uses internally over 200 DSLs).

A particular flavor of DSLs are internal or embedded DSLs which can
seamlessly inter-operate with the underlying (typically general-purpose)
language. However, internal DSLs offer only limited range of syntax
and are typically not supported by IDEs. Contrary to this, external
DSLs admit almost any syntax, and modern DSL engineering tools (like
MPS \citep{campagne2016themps}, Xtest \citep{bettini2016implementing},
textX \citep{dejanovic2017textxa}, or Spoofax \citep{kats2010thespoofax})
provide ``automatic'' editing support tools (syntax checking and
code completion) for them. The disadvantage of external DSLs is the
difficulty of interaction with (general-purpose) languages. Paired
with this is increased development effort in a scenario where DSL
capabilities are not sufficient, and e.g. writing project-specific
User Defined Functions become necessary.

In our approach we generate code for a general-purpose language from
an external DSL during the editing process, which largely eliminates
the interoperability barrier. We also implemented a special Language
Server to provide coding assistance to both our DSL and the ``embedding''
general-purpose language (here Python).


==> latex mirror/060-conclusions.tex <==

\section{Conclusions and Future Work} \label{sec:Future-Work-and-Conclusions}

We proposed a DSL-based approach to support data scientists in writing
code for common tasks related to table analysis and processing. We
use external DSL to express such operations in a human-readable form,
and generate executable Python code directly during editing. In this
way we circumvent the frequently encountered problem of insufficient
expressiveness of a DSL, since developers can directly use Python
code to address more special cases (outside the power of the DSL).
Our prototype works with a large number of IDEs and editors (all supporting
the Language Server Protocol), and provides editing support (code
recommendations) for the DSL.

Moreover, users can generate code for Pandas ``data wrangling''
library, or for Apache Spark. This facilitates a transition from low-effort
yet typically non-scalable scripts (in Pandas) suitable for smaller
data sets to highly scalable scripts in Spark. Our preliminary evaluation
shows that for typical data pre-processing tasks, our DSL is capable
of generating complete code in 10 out of 16 cases for Apache Spark,
and in 9 out of 14 cases for Pandas.

Despite of these promising results, there is still a lot of work to
be done to understand and to address the challenges of our approach,
and to provide tools of practical value. Our future work will include
a controlled user study with interviews in order to identify such
challenges, and verify our hypotheses on user behavior. We will also
implement more code generation targets for our DSL, including R (with
dplyr/tidyR) and Matlab. Another option is to provide and evaluate
a DSL for deep learning frameworks like TensorFlow, Microsoft Cognitive
Toolkit, or PyTorch.

Further work related to the editing support will include mechanisms
for synchronizing DSL and the generated code, e.g. by marking DSL
code which is no longer in-sync with the Python code. Another option
here is to add support for ``type providers'' known from .NET languages,
i.e. editor/compiler recommendations for column names and types of
the actual data sets processed in a script.



